Gaussian Process Bandits with Aggregated Feedback

We consider the continuum-armed bandits problem, under a novel setting of recommending the best arms within a fixed budget under aggregated feedback. This is motivated by applications where the precise rewards are impossible or expensive to obtain, while an aggregated reward or feedback, such as the average over a subset, is available. We constrain the set of reward functions by assuming that they are from a Gaussian Process and propose the Gaussian Process Optimistic Optimisation (GPOO) algorithm. We adaptively construct a tree with nodes as subsets of the arm space, where the feedback is the aggregated reward of representatives of a node. We propose a new simple regret notion with respect to aggregated feedback on the recommended arms. We provide theoretical analysis for the proposed algorithm, and recover single point feedback as a special case. We illustrate GPOO and compare it with related algorithms on simulated data.

==> sections/special_case_S1.tex <==
\subsection{Regret Bound for special case $S=1$}
\label{app:s=1}

\begin{lemma}
\label{lemma: on event xi Ih}
Suppose $S=1$, implying that any cell $\mathcal{X}_{h,i}$ possesses only one representative point $\bm{x}_{h,i}$. On the event $\xi$, GPStoOO only expands nodes that belong to the set $I:= \cup_{h \geq 0} I_h$, where $I_h:= \{(h,i)| f\left(\bm{x}_{h, i}\right) + 3 \delta(h) \geq f^\ast\}.$
\end{lemma}

\begin{proof}
Let $(h_t, j_t)$ be the node expanded at time $t$. 
We know from Algorithm \ref{alg: GPOO}, the b-value of $h_t, j_t$ is larger than or equal to the b-value of the cell $h_t^\ast, j_t^\ast$ containing $\bm{x}^\ast$.
Then under event $\xi$,
\begin{align*}
  &\phantom{{}\geq}f\left(\bm{x}_{h_t, j_t}\right) \\
  &\geq \mu(X_{h, j} \mid Z_{t-1}) - CI_t(X_{h,j} ) && \text{Lemma}~\ref{lemma: tail bound on event xi}\\
  &= b_{h_{t}, j_{t}}(t)- 2CI_t(X_{h,j} ) - \delta\left(h_{t}\right)&& \text{By } \eqref{equ: b-value of GPOO}\\
  &\geq b_{h_{t}^{*}, j_{t}^{*}}(t)-3 \delta\left(h_{t}\right) && \text{Algorithm } \ref{alg: GPOO} , \text{ line }7,3\\
  &\geq f\left(\bm{x}_{h_{t}^{*}, j_{t}^{*}}\right) +\delta\left(h_{t}^{*}\right)-3 \delta\left(h_{t}\right) && \text{By } \eqref{equ: b-value of GPOO} \text{, on event } \xi\\ 
  & \geq f\left(\bm{x}_{h_{t}^{*}, j_{t}^{*}}\right) + L \sup_{\bm{x} \in X_{h_{t}^{*}, j_{t}^{*}}} \ell(\bm{x}_{h_{t}^{*}, j_{t}^{*}}, \bm{x})-3 \delta\left(h_{t}\right) && \text{By Assumption }\ref{ass: decreasing diameters} \\
  & \geq f\left(\bm{x}_{h_{t}^{*}, j_{t}^{*}}\right) + L \ell(\bm{x}_{h_{t}^{*}, j_{t}^{*}}, \bm{x}^\ast) -3 \delta\left(h_{t}\right) && \bm{x}^\ast \in X_{h_{t}^{*}, j_{t}^{*}}\\ 
  & \geq f^{*}-3 \delta\left(h_{t}\right) && \text{By Lemma } \ref{lemma: tail bound on event xi}
\end{align*}
\end{proof}


We bound the number of nodes in $I_h$ by the near-optimality dimension.

\begin{lemma}
\label{lemma: upper bound of Ih GPOO S=1}
Recall $d^{\eta, \ell}$ be the ${\eta, \ell}-$near-optimality, and $C$ be the corresponding constant. Then under Assumption \ref{ass: well-shaped cells},
\begin{align}
  |I_h| \leq C [3 \delta(h)]^{-d^{\eta, \ell}}.
\end{align}
\end{lemma}

  \begin{proof}
    From Lemma \ref{lemma: on event xi Ih}, we know $I_h$ is the set of nodes at depth $h$ such that the point with maximum function value in that node is within $3 \delta(h)$ of the optimal state. That is, 
    \begin{align*}
      |I_h| &= |\{(h,i)|f\left(\bm{x}_{h, j}\right) \geq f^\ast - 3 \delta(h)\}|\\
        &= |\bm{x}_{h,i} \in \mathcal{X}_{3\delta(h)}|.
    \end{align*}
    From Assumption \ref{ass: well-shaped cells}, 
    if $|\{(h,i)|\bm{x} \in \mathcal{X}_{3 \delta(h)} \}| > C [3 \delta(h)]^{-d^{\eta, \ell}}$, 
    there exists at least more than $C [3 \delta(h)]^{-d^{\eta, \ell}}$ disjoint $\ell-$ball of radius $\nu \delta(h)$, which contradicts the definition of $d^{\eta, \ell}$ (Definition \ref{defi: near-optimality dimension}, take $\epsilon = 3 \delta(h)$).
    Chaining these together, we have $|I_h| \leq C [3 \delta(h)]^{-d^{\eta, \ell}}$.
  \end{proof}


\begin{theo}
Define $h_N$ as the smallest integer $h^\prime$ up to round $N$ such that 
\begin{align}
\label{equ: GPOO loss bound hn defi centre}
  \frac{N}{\beta_{N}} \leq K \sum_{h = 0}^{h'} C [3 \delta(h)]^{-d^{\nu, \delta}} \frac{\sigma^2}{\delta^2(h)}
\end{align}

For constant $a$ specified in Lemma \ref{lemma: tail bound on event xi}, and $\delta \in (0, 1 - a)$, with probability of $1-\delta-a$, the simple regret of GPOO is bounded as 
\begin{align}
  R_N \leq 3 \delta(h_N).
\end{align}
\end{theo}

\begin{proof}
  Let $T_{X_{h, \cdot}}(N)$ be the number of times a node at depth $h$ has been evaluated up to round $N$. 
  We consider two types of nodes in terms of whether the nodes have been expanded at round $N$. 
  According to Lemma \ref{lemma: on event xi Ih}, for all nodes at level $h \in [0, h_{\max}]$,
  nodes that have been expanded belong to $I_h$ under event $\xi$;
  for those who have not been expanded, we track them according to their parents (which belong to $I_{h-1}$).
  Then by Lemma \ref{lemma: upper bound of Ih GPOO S=1} \text{ and } \ref{lemma: upper bound for number of draws average}, we have
  \begin{align*}
      N \leq& \sum_{h=0}^{h_{\max }}\left|I_{h}\right| T_{X_{h, \cdot}}(N) +(K-1) \sum_{h=1}^{h_{\max }+1}\left|I_{h-1}\right| T_{X_{h-1, \cdot}}(N)\\
      % =& K \sum_{h = 0}^{h_{\max}} |I_h| T_{h}(N)\\
      \leq& K \sum_{h = 0}^{h_{\max}} C [3 \delta(h)]^{-d^{\eta, \ell}}
      \frac{\beta_{N+1} \sigma^2}{\delta^2(h)}.
  \end{align*}
  From E.q. (\ref{equ: GPOO loss bound hn defi ave}), we know that $h_N \leq h_{\max}$, and from Algorithm \ref{alg: GPOO} and Lemma \ref{lemma: on event xi Ih},
  \begin{align*}
      \bar{F}(X_{N}) \geq f^\ast - 3 \delta(h_{\max})  \geq f^\ast - 3 \delta(h_N),
  \end{align*}
  where $X_{N}$ is the recommended cell at round $N$. Thus, 
  \begin{align*}
      R_N = f^\ast - \bar{F}(X_N) \leq 3 \delta(h_N).
  \end{align*}
\end{proof}
  



% \section{Proofs of Gaussian process properties}
\iffalse
\begin{lemma}
  \label{lemma: uni_gauss_conc}
  Pick $\delta \in(0,1)$ and set $\beta_{t}=$ $2 \log \left(N \pi_{t} / \delta\right)$,
  % where $\sum_{t \geq 1} \pi_{t}^{-1}=1, \pi_{t}>0 .$
  where $\pi_{t}=\pi^{2} t^{2} / 6$.
  % REVIEW: other choices of pi?
  Then
  $$
  \left|f(S)-\mu_{t-1}(S)\right| \leq \beta_{t}^{1 / 2} \sigma_{t-1}(S) \quad \forall S \in \mathcal{G}^\ast \quad \forall t \geq 1
  $$
  holds with probability $\geq 1-\delta$.
\end{lemma}

\begin{proof}
  Fix $t \geq 1$ and $S \in \mathcal{G}_\ast$. Conditioned on $\bm{y}_{\widetilde{\mathcal{S}}_{t-1}} = \{y_{S_1}, \dots, y_{S_{t-1}}\}, \{S_1, \dots, S_N\}$ are deterministic,
  % \textcolor{red}{why do we need that sentence (copied from \cite{srinivas2009_GPUCB})?} \russ{If they are not deterministic, unless I am mistaken, the distribution of $f(S)$ is highly non trivial and no longer Gaussian.}
  and $f(S) \sim \mathcal{N}(\mu_{t-1}(S), \sigma^2_{t-1}(S))$.
  If $r \sim \mathcal{N}(0,1)$, then
  \begin{align}
      \operatorname{Pr}\{r>c\}
      &= \int_c^\infty \frac{1}{\sqrt{2 \pi}} e^{r^2/2} d r \\
      &=e^{-c^{2} / 2}\frac{1}{\sqrt{2 \pi}} \int_c^\infty e^{-\frac{(r-c)^2}{2}-c(r-c)} d r\\
      &\leq e^{-c^{2} / 2}\frac{1}{\sqrt{2 \pi}} \int_c^\infty e^{-\frac{(r-c)^2}{2}} d r && e^{-c(r-c)} \leq 1 \text{ for } r \geq c \text{ and } c>0\\
      &= e^{-c^{2} / 2} \operatorname{Pr}\{r>0\}=(1 / 2) e^{-c^{2} / 2}
  \end{align}

  Therefore, using $r=\left(f(S)-\mu_{t-1}(S)\right) / \sigma_{t-1}(S)$ and $c=\beta_{t}^{1 / 2}$,
  $$
  \operatorname{Pr}\left\{\left|f(S)-\mu_{t-1}(S)\right| > \beta_{t}^{1 / 2} \sigma_{t-1}(S)\right\} \leq e^{-\beta_{t} / 2},
  $$
  Applying
  the union bound,
  $$
  \left|f(S)-\mu_{t-1}(S)\right| \leq \beta_{t}^{1 / 2} \sigma_{t-1}(S) \quad \forall S \in \mathcal{G}^\ast
  $$
  holds with probability $\geq 1-N e^{-\beta_{t} / 2}$. Choosing $N e^{-\beta_{t} / 2}=\delta / \pi_{t}$ and using the union bound for $t \in \mathbb{N}$, the statement holds. For example, we can use $\pi_{t}=\pi^{2} t^{2} / 6$.
\end{proof}
\fi

